Ramsey Quantifiers over Automatic Structures: Complexity and Applications to Verification

Automatic structures are infinite structures that are finitely represented by synchronized finite-state automata. This paper concerns specifically automatic structures over finite words and trees (ranked/unranked). We investigate the "directed version" of Ramsey quantifiers, which express the existence of an infinite directed clique. This subsumes the standard "undirected version" of Ramsey quantifiers. Interesting connections between Ramsey quantifiers and two problems in verification are firstly observed: (1) reachability with B\"{u}chi and generalized B\"{u}chi conditions in regular model checking can be seen as Ramsey quantification over transitive automatic graphs (i.e., whose edge relations are transitive), (2) checking monadic decomposability (a.k.a. recognizability) of automatic relations can be viewed as Ramsey quantification over co-transitive automatic graphs (i.e., the complements of whose edge relations are transitive). We provide a comprehensive complexity landscape of Ramsey quantifiers in these three cases (general, transitive, co-transitive), all between NL and EXP. In turn, this yields a wealth of new results with precise complexity, e.g., verification of subtree/flat prefix rewriting, as well as monadic decomposability over tree-automatic relations. We also obtain substantially simpler proofs, e.g., for NL complexity for monadic decomposability over word-automatic relations (given by DFAs).

==> app-recognizable.tex <==
\begin{lemma}\label{lem:hardness}
Given a binary regular relation $R \subseteq \Sigma^* \times \Sigma^*$ by an NFA (resp. DFA),
it is $\PSPACE$-hard (resp. $\NL$-hard) to decide whether $R$ is monadically decomposable.
Given a binary tree-regular relation $R \subseteq \T_\Sigma \times \T_\Sigma$ by an NTA (resp. D$\uparrow$TA),
it is $\EXP$-hard (resp. $\P$-hard) to decide whether $R$ is monadically decomposable.
\end{lemma}
\begin{proof}
We give a logspace reduction from the universality problem which is known to be $\PSPACE$-complete for NFAs,
$\NL$-complete for DFAs, $\P$-complete for D$\uparrow$TAs, and $\EXP$-complete for NTAs.
In the following we only consider the word case.
Recall that the universality problem asks whether for a given regular language $L \subseteq \Sigma^*$ it holds that $L = \Sigma^*$.
Let $L \subseteq \Sigma^*$ be a regular language given by an NFA (resp. DFA) $\A$.
We define the regular relation
\[R_L := \{(u \otimes v, w) \mid u \in L \text{ or } v = w \in \Sigma^*\}.\]
It is easy to construct an NFA (resp. DFA) that recognizes $R_L$ in logarithmic space from $\A$. 
Note that for DFAs the disjunction can be realized with a product construction.
It remains to show that $R_L$ is monadically decomposable if and only if $L = \Sigma^*$.

If $L = \Sigma^*$, it holds that $R_L = \{(u \otimes v, w) \mid u,v,w \in \Sigma^*\}$ which is clearly monadically decomposable.

For the converse assume that there exists $u_0 \in \Sigma^* \setminus L$.
Then the intersection of $R_L$ with the monadically decomposable relation 
$\{(u_0 \otimes v, w) \mid v,w \in \Sigma^*\}$
is the relation
$\{(u_0 \otimes v, w) \mid v = w \in \Sigma^*\}$,
which is not monadically decomposable.
Since monadically decomposable relations are closed under intersection, it follows that $R_L$ is not monadically decomposable.
\end{proof}

\begin{lemma}\label{lem:det-hard}
Given a binary tree-regular relation $R \subseteq \T_\Sigma \times \T_\Sigma$ by a D$\downarrow$TA,
it is $\P$-hard to decide whether $R$ is monadically decomposable.
\end{lemma}
\begin{proof}
We give a logspace reduction from the emptiness problem for D$\downarrow$TAs which is known to be $\P$-complete \cite{veanes1997computational}. 
Let $\A = (Q,\Sigma,\Delta,q_0)$ be a D$\downarrow$TA. 
We construct a D$\downarrow$TA $\A' = (Q,\Gamma_\bot^2,\Delta',q_0)$ recognizing a binary tree-regular relation $R'$ over 
$\Gamma := \Sigma \cup \{\#\}$ where $\# \notin \Sigma$ is a symbol of rank 1 as follows. 
We define the transition relation $\Delta'$ such that
\begin{itemize}
\item $q \xrightarrow{(a,a)}_{\A'} (q_1,\dots,q_r)$ for all $q \xrightarrow{a}_{\A} (q_1,\dots,q_r)$,
\item $q_0 \xrightarrow{(\#,\#)}_{\A'} q_0$
\end{itemize}
Clearly, $\A'$ can be constructed in logspace from $\A$.

It is easy to see that $R' \subseteq \{(t,t) \mid t \in \T_{\Gamma}\}$. 
Moreover, it holds that $R'$ is finite if and only if $L(\A) = \emptyset$.  
Indeed, if there exists $t \in L(\A)$, then $(t_n,t_n) \in R'$ for all $n \geq 0$ 
where $t_n$ is the resulting tree when padding a chain of $\#$-symbols of length $n$ to the root of $t$. 
Since every finite relation is monadically decomposable and every infinite subrelation of $\{(t,t) \mid t \in \T_{\Gamma}\}$ is clearly not monadically decomposable, 
it holds that $R'$ is monadically decomposable if and only if $L(\A) = \emptyset$.
\end{proof}


